Quilt-1M: One Million Image-Text Pairs for Histopathology

Recent accelerations in multi-modal applications have been made possible with the plethora of image and text data available online. However, the scarcity of analogous data in the medical field, specifically in histopathology, has slowed comparable progress. To enable similar representation learning for histopathology, we turn to YouTube, an untapped resource of videos, offering $1,087$ hours of valuable educational histopathology videos from expert clinicians. From YouTube, we curate QUILT: a large-scale vision-language dataset consisting of $802, 144$ image and text pairs. QUILT was automatically curated using a mixture of models, including large language models, handcrafted algorithms, human knowledge databases, and automatic speech recognition. In comparison, the most comprehensive datasets curated for histopathology amass only around $200$K samples. We combine QUILT with datasets from other sources, including Twitter, research papers, and the internet in general, to create an even larger dataset: QUILT-1M, with $1$M paired image-text samples, marking it as the largest vision-language histopathology dataset to date. We demonstrate the value of QUILT-1M by fine-tuning a pre-trained CLIP model. Our model outperforms state-of-the-art models on both zero-shot and linear probing tasks for classifying new histopathology images across $13$ diverse patch-level datasets of $8$ different sub-pathologies and cross-modal retrieval tasks.

==> sections/7_checklist.tex <==


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/dump.tex <==

%-------------------------------------------------------------------------

%OTHER RELEVANT PAPERS INTRODUCTION SETUP
%LN:
%Introduction:
%-The need for grounded multimodal data
%-Thier data contribution (hig-level)
%- Their dataset curation details (high level)
%- Benefits of their curation process (cost, speed, size, richness, automated nature), over other similar datasets
%- Data Characteristics
%- Main Tasks enabled by thier data
%- other posible tasks (side tasks)
%- summarized list of contributions

%Details abpout the dataset form the annotation process, to data characteristics and statistics, to dtat sources  and localization accuracy, to the 

%Controlled Image captioning

%Ablation of adding trace or ROI


%BiomedClip:
%Introduction:
%- Use of multimodal data on the state of art in varying tasks
%- limitations in medical
%- data contribution high-level
%- detailed contribution


%ARCH
%Introduction:
%- Use/need for data in represnetation data
%- recent works/success of NN in computational pathology
%- advances in weak or unsupervised rep learning
%- massive demand for pretrained pathology rep model
%- rep learning through image captioning
%- properties of the arch data
%- comparisms against natural image -text datasets and how they provide more reprsentation power thann unimodal data like imagenet, and how in this histo context arch fits better
%- sumarry of contributions


- Start with how difficult it is to collect medical dataset, especially multimodal datasets that require tons of time and high level expertise. It therefore necessary to find sources of data (psuedo) to leverage

- Talk about how in pathology its hard to get multimodal data outside of pathology reports which in many cases could provide a single sentence to communicate findings in a set of WSIs for patient one of which could be an image thats 200K by 100K in size, and hence theres is inherent imbalance.

- Introduce the dataset its novelty in terms of modalities, range of sub-pathology types, the magnitude/scales present and pipeline to collect it from open/available videos.

-make similar claims like arch on the inprotance of having a dataset by which to pretrain in-domain histopathology encoders for downstream histology tasks, esp with the boom in computational histopathology in recent years

- talk little about how it compares to arch in structure and size. by structure I mean is more noisy, however, contains more information about WSI case from macro level down to the patches, and hance provides more information which if learned in pretraining could be very beneficial for downstream tasks. Also talk about the size of our dataset which id X times larger in size (pairs) and also contains multiple text per image, unlike Arch that has multiple images for one text, make our dataset more on par with COCO

- finally mention how our method is generalizable to many other medical domains and evn non-medical domains.

- captures WSI as a set of unrolled patches much like unrolling a video 

true few-shot, vanilla In-context learning


%use table to show that data that goes into model, talk about the patching into images of varying scales and sizes to improve generalization, also touch on the choice of tcga subset , and the addtion of patch only cytology and IHC stain image to improve generalizabilty.

give brief decrition of training parameters and model architecture

detail of magni model training, data, model achritecture






Although our process for cropping the relevant images can be noisy and hence still produce artefact in the image this can be greatly reduced by providing grounded spatial context using ROI during pretraining. E.g A histopathology image with some text or blob artifacts on the image may constitute noise/spurious information, however, cursor movement on the relevant parts of the image if utilized draw attention to useful information of the image.

- Cursor tracking: (add resons why its a hard problem due to variance of cursor types), use of domain knowledge of absdiff of static scenes to find cursor


%ToDo
%-  To prevent GPT from haullicination we provide few shot examples that do not have any correction, medical text or roi text, several examples are discussed in the appendix.

% - put description of histo classifier in supplementary and just cite it in the main

% add ACRO dataset to table 5 of datasets used to train histoclf

%- tomorrow when you have time can you write the zero shot part very shortly under section 5 for algorithmic details. Like how did we use the templates, when used 4 templates how did we average it etc. (edited) 

%-update downstream dataset tabzle in supplementary

% go over Appendix/Supplementary, FIgures, captions, labels, 

%add acc of classifer






% FULL LINEAR PROBE TABLE WITH MHIST, WHICH IS REMOVED ON THE MAIN PAPER
\begin{table}[!ht]
\centering
%\footnotesize
\tablestyle{0.3pt}{1.0}
\begin{tabular}{lc|cc>{\columncolor{defaultcolor}}c|c>{\columncolor{defaultcolor}}cc>{\columncolor{defaultcolor}}c}
\toprule
 \multirow{2}{*}{Dataset} &  \multirow{3}{*}{\%-shot}  & \multicolumn{3}{c|}{ViT-B/32}  & \multicolumn{4}{c}{ViT-B/16} \\
\cmidrule(lr){3-9}
         &        & CLIP   &   PLIP   & \ourmodel{} & CLIP   &   \ourmodel{} &   BiomedCLIP  &  \ourmodel{}   \\
 Supervised (\%)       &        & GPT/77 &  GPT/77  &   GPT/77    & GPT/77 &    GPT/77      &    PMB/256     &   PMB/256      \\
 \shline
\multirow{2}{*}{NCT-CRC }& 1    & 91.0 (0.10) & 93.75 (0.09) & \textbf{94.64}(0.22) & 90.96 (0.10) &  93.36 (0.23) & 92.14 (0.12) &  \textbf{93.55} (0.25)  \\
                         & 10   & 92.02 (1.30) & 93.83 (0.06)	& \textbf{95.30} (0.03) & 92.58 (0.12) &  \textbf{93.85} (0.04) & 92.90 (0.07) & 93.72 (0.08)   \\
      (94.0)             & 100  & 91.83 (0.01) & 94.16 (0.01)	& \textbf{95.22} (0.01) & 92.26 (0.09) &  \textbf{93.76} (0.02) & 92.97 (0.05) & 93.60 (0.01)    \\
\cmidrule(lr){1-9}
\multirow{2}{*}{PatchCamelyon} & 1 & 80.38 (0.16) & 87.26 (0.23) & \textbf{87.62} (0.35) & 80.28 (0.20) &  \textbf{84.78} (0.14) & 83.63 (0.44) & 83.48 (0.18)   \\
                         & 10   & 82.67 (0.19) & 87.48 (0.08) & \textbf{87.55} (0.03) & 82.20 (0.04) &  \textbf{86.77} (0.09) & 84.18 (0.15) & 84.42 (0.10)     \\
       (97.5)                  & 100  & 82.80 (0.01) & 87.34 (0.01) & \textbf{87.48} (0.01) & 82.55 (0.02) &  \textbf{86.81} (0.04) & 84.23 (0.01) & 84.44 (0.02)     \\
\cmidrule(lr){1-9}
\multirow{2}{*}{SkinCancer} & 1   & 84.27 (0.22) & \textbf{91.07} (0.25) & 90.93 (0.25) & 85.62 (0.16) &  \textbf{88.29} (0.15) & 87.53 (0.21)  & 88.06 (0.20)  \\
                         & 10   & 89.0 (0.02)  & \textbf{93.39} (0.05)	& 92.99 (0.02) & 90.28 (0.01) &  \textbf{91.20} (0.0) & 89.23 (0.03) & 90.03 (0.02)    \\
        (93.3)                 & 100  & 89.02 (0.02) & \textbf{93.29} (0.01) & 93.03 (0.02) & 90.29 (0.03) &  \textbf{91.20} (0.0) & 89.16 (0.02) & 89.91 (0.01)     \\
\cmidrule(lr){1-9}
% \multirow{2}{*}{MHIST}      & 1    & 64.35 (2.88) & \textbf{66.35} (0.41) & 63.25 (2.77) & 63.43 (2.28) &  60.66 (1.02) & \textbf{68.88} (1.94)  & 67.93 (1.70)    \\
%                          & 10   & 68.88 (2.52) & \textbf{71.10} (1.34) & 67.65 (0.90) & \textbf{78.33} (2.59) &  67.01 (1.84) & 74.34 (1.22) & 73.63 (1.10)    \\
%        (85.1)                  & 100  &  \textbf{75.91} (0.46) & 74.21 (0.30) & 74.68 (0.46) & 73.86 (0.17) &  73.73 (0.21) & \textbf{78.30} (0.33) & 76.46 (0.14)     \\
% \cmidrule(lr){1-9}
\multirow{2}{*}{SICAPv2}    & 1    & 52.45 (2.41) & 65.76 (2.65) & \textbf{69.92} (1.02) & 56.01 (0.66) &  66.86 (1.16) & \textbf{69.43} (1.03) & 68.49 (1.06)  \\	
                         & 10   & 62.24 (0.65) & 69.23 (0.43) & \textbf{74.14} (0.38) & 63.70 (0.69) &  72.37 (0.65) & 71.61 (0.31) & \textbf{72.48} (0.42)    \\
       (67.0)                  & 100  & 65.75 (0.16) & 73.0 (0.14) & \textbf{75.48} (0.12) & 68.74 (0.10) &   74.14 (0.16) & 74.57 (0.04) & \textbf{74.60} (0.17)   \\
\shline
\end{tabular}
\caption{Linear probing image classification. accuracy (\%) * trained from scratch. SkinTumor is the Neoplastic Subset of SkinCancer, NCK here is without the BACK label which is easily discriminatory \cite{ikezogwo2022multi}}
\label{tab:zeroshot}
\end{table}
























%#########################    Cross retrieval results       ###################


















\begin{table}[!ht]
\centering
\tablestyle{1.5pt}{1.1}
\begin{tabular}{ll|rrrrr|rrrrr}
\toprule
\multicolumn{12}{c}{Quilt: Holdout Set}  \\
\toprule
& & \multicolumn{5}{c|}{Text-to-Image (\%)} & \multicolumn{5}{c}{Image-to-Text (\%)} \\
\cmidrule(lr){3-12}
model & config & R@1 & R@5 & R@10 & R@50 & R@200 & R@1 & R@5 & R@10 & R@50 & R@200 \\
 \shline
CLIP                                & ViT-B/32|GPT/77 & 0.49 & 1.28 & 2.01 & 4.73 & 10.15 & 0.39 & 1.01 & 1.56 & 3.99 & 8.80  \\
PLIP                                & ViT-B/32|GPT/77 & 1.05 & 3.20 & 4.83 & 10.79 & 21.80 & 0.87 & 2.98 & 4.62 & 11.04 & 21.63 \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/32|GPT/77 & \textbf{1.17} & \textbf{3.84} & \textbf{6.09} & \textbf{16.31} & \textbf{31.99} & \textbf{1.24} & \textbf{3.98} & \textbf{6.02} & \textbf{14.89} & \textbf{28.97} \\
\cmidrule(lr){1-12}
CLIP                                & ViT-B/16|GPT/77 & 0.83 & 1.67 & 2.34 & 5.63 & 11.26 & 0.66 & 1.47 & 2.04 & 5.02 & 10.82  \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/16|GPT/77 & 2.42 & 6.23 & 9.44 & 22.38 & 41.05 & 2.00 & 5.87 & 8.83 & 21.66 & 39.29  \\
BiomedCLIP                          & ViT-B/16(224)|PMB/256 &  4.34 & 7.08 & 8.77 & 14.99 & 25.62 & 3.88 & 6.64 & 8.21 & 13.93 & 23.53  \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/16(224)|PMB/256 & \textbf{6.20} & \textbf{11.95} & \textbf{15.90} & \textbf{30.28} & \textbf{50.60} & \textbf{6.27} & \textbf{12.48} & \textbf{16.43} & \textbf{31.06} & \textbf{50.86}  \\
\end{tabular}
\caption{Cross-modal retrieval results on \ourdata{} test set.}
\label{tab:txt-img}
\end{table}


\begin{table}[!ht]
\centering
\tablestyle{1.5pt}{1.1}
\begin{tabular}{ll|rrrrr|rrrrr}
\toprule
\multicolumn{12}{c}{ARCH}  \\
\toprule
& & \multicolumn{5}{c|}{Text-to-Image (\%)} & \multicolumn{5}{c}{Image-to-Text (\%)} \\
\cmidrule(lr){3-12}
model & config & R@1 & R@5 & R@10 & R@50 & R@200 & R@1 & R@5 & R@10 & R@50 & R@200 \\
 \shline
CLIP                                & ViT-B/32|GPT/77 & 0.07 & 0.41 & 0.74 & 2.42 & 7.21 & 0.05 & 0.34 & 0.70 & 2.52 & 7.22  \\
PLIP                                & ViT-B/32|GPT/77 & 0.56 & 2.56 & 4.45 & 13.10 & 29.85 & 0.74 & 2.88 & 4.56 & 13.75 & 29.46 \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/32|GPT/77 & \textbf{1.41} & \textbf{4.96} & \textbf{7.57} & \textbf{19.87} & \textbf{39.13} & \textbf{1.35} & \textbf{4.54} & \textbf{7.62} & \textbf{19.20} & \textbf{38.57} \\
\cmidrule(lr){1-12}
CLIP                                & ViT-B/16|GPT/77 & 0.09 & 0.47 & 0.77 & 2.73 & 8.72 & 0.13 & 0.49 & 0.81 & 3.09 & 9.04  \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/16|GPT/77 & 1.29 & 4.89 & 7.66 & 20.30 & 40.89 & 1.01 & 3.68 & 5.56 & 16.18 & 34.15  \\
BiomedCLIP                          & ViT-B/16(224)|PMB/256 & \textbf{8.89} & \textbf{22.84} & \textbf{31.22} & 53.24 & 71.43 & \textbf{9.97} & \textbf{24.26} & \textbf{32.28} & 52.13 & 68.47  \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/16(224)|PMB/256 & 8.77 & 21.67 & 30.17 & \textbf{55.14} & \textbf{77.64} & 9.85 & 23.59 & 31.42 & \textbf{53.06} & \textbf{73.43}  \\
\end{tabular}
\caption{Cross-modal retrieval results on ARCH dataset.}
\label{tab:txt-img-arch}
\end{table}





\begin{table}[!ht]
\centering
\tablestyle{0.8pt}{1.}
\begin{tabular}{ll|rrr|rrr||rrr|rrr}
\toprule
& & \multicolumn{3}{c|}{Text-to-Image (\%)} & \multicolumn{3}{c}{Image-to-Text (\%)} & \multicolumn{3}{c|}{Text-to-Image (\%)} & \multicolumn{3}{c}{Image-to-Text (\%)} \\
\cmidrule(lr){3-12}
model & config & R@1 & R@50 & R@200 & R@1 & R@50 & R@200 & R@1 & R@50 & R@200 & R@1 & R@50 & R@200 \\
 \shline
CLIP                                & ViT-B/32|GPT/77 & 0.49 &  4.73 & 10.15 & 0.39 & 3.99 & 8.80  & 0.07 & 2.42 & 7.21 & 0.05 &  2.52 & 7.22  \\
PLIP                                & ViT-B/32|GPT/77 & 1.05 & 10.79 & 21.80 & 0.87 & 11.04 & 21.63  & 0.56 & 13.10 & 29.85 & 0.74 & 13.75 & 29.46 \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/32|GPT/77 & \textbf{1.17} & \textbf{16.31} & \textbf{31.99} & \textbf{1.24} & \textbf{14.89} & \textbf{28.97} & \textbf{1.41} &  \textbf{19.87} & \textbf{39.13} & \textbf{1.35} & \textbf{19.20} & \textbf{38.57} \\
\cmidrule(lr){1-12}
CLIP                                & ViT-B/16|GPT/77 & 0.83 &  5.63 & 11.26 & 0.66 & 5.02 & 10.82  & 0.09 &  2.73 & 8.72 & 0.13 & 3.09 & 9.04  \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/16|GPT/77 & 2.42 &  22.38 & 41.05 & 2.00 &  21.66 & 39.29  & 1.29 &  20.30 & 40.89 & 1.01 & 16.18 & 34.15  \\
BiomedCLIP                          & ViT-B/16|PMB/256 &  4.34 & 14.99 & 25.62 & 3.88 & 13.93 & 23.53  & \textbf{8.89} &  53.24 & 71.43 & \textbf{9.97} & 52.13 & 68.47  \\
\rowcolor{defaultcolor}\ourmodel{}  & ViT-B/16|PMB/256 & \textbf{6.20} &  \textbf{30.28} & \textbf{50.60} & \textbf{6.27} & \textbf{31.06} & \textbf{50.86}  & 8.77 & \textbf{55.14} & \textbf{77.64} & 9.85 &\textbf{53.06} & \textbf{73.43}  \\
\end{tabular}
\caption{Cross-modal retrieval results on \ourdata{} test set.}
\label{tab:txt-img}
\end{table}






\begin{tcbraster}[raster columns=3,raster equal height,nobeforeafter,raster column skip=0.5cm]
  \begin{tcolorbox}[title=box 1]
    apple
  \end{tcolorbox}
  \begin{tcolorbox}[title=box 2]
    peach
  \end{tcolorbox}
  \begin{tcolorbox}[title=box 3]
    banana
  \end{tcolorbox}
\end{tcbraster}
\begin{tcbraster}[raster columns=3,raster equal height,nobeforeafter,raster column skip=0.5cm]
  \begin{tcolorbox}[title=box 4]
    pear
  \end{tcolorbox}
  \begin{tcolorbox}[title=box 5]
    cherry
  \end{tcolorbox}
  \begin{tcolorbox}[title=box 6]
    grape
  \end{tcolorbox}
\end{tcbraster}














\subsubsection{Filtering for Narrative-Style Medical Videos}
\label{search_filter}


Non-voiced videos are also filtered by using inaSpeechSegmenter \cite{ddoukhanicassp2018} in instances where the video endpoint does not return the video language or transcript. To identify a video's audio language, we first check YouTube's API, and if unavailable, we use OpenAI's Whisper model \cite{radford2022robust} on the video's first minute of audio.

For all videos meeting these heuristics, two decisions are made:
%\renewcommand{\labelenumi}{\alph{enumi}} 
\begin{enumerate}[label=(\Alph*)]
    \item Do they have the required medical content, i.e., histopathology image-text pairs?
    \item If so, are they in narrative style -- videos wherein the presenter(s) spend a significant time panning and zooming on parts or the entire whole slide image while providing vocal descriptions of image content?
\end{enumerate}  

% For all videos that meet the set heuristics, we need to determine two things:
% %\renewcommand{\labelenumi}{\alph{enumi}} 
% \begin{enumerate}[label=(\Alph*)]
%     \item Do they have the required medical content i.e, histopathology image-text
%     \item If so, are they in narrative style -- videos wherein the presenter(s) spends significant time panning and zooming on parts or the whole slide image while providing vocal description of image content.
% \end{enumerate}  

To automatically identify the relevant videos, we first extract key frames from a video. These key frames are automatically extracted using FFmpeg \footnote{https://ffmpeg.org/}, marking the beginning or end of a scene. Scene frames denote frames containing insignificant visual changes given a threshold that determines the minimum amount of visual change required to trigger a scene frame. Through experimentation, we set different thresholds for various video durations, with smaller thresholds for longer videos. We then linearly interpolate for new video durations to set its threshold, with the lowest threshold being $0.008$ (5-minute video) and the highest $0.25$ (200-minute video).

% To find these video automatically, first, we extract scene frames from the video, these are key frames automatically extracted using FFmpeg \footnote{https://ffmpeg.org/} that mark the beginning or end of a scene (frames that contain insignificant visual changes) given a threshold that determines the minimum amount of visual change required to trigger a scene frame, which can be useful for tasks such as video summarization, indexing, or content-based retrieval. Through experimentation we set different, decreasingly smaller, thresholds for increasing video durations and linearly interpolate for new video duration's to set its threshold, with the lowest threshold being $0.008$ (5-minute video) and the highest $0.25$ (200-minute video).

%## add the emsemble histo classifier and change Do they have wisdom

% For \textbf{(A)} we trained a set of binary image classifiers and ensemble their predictions to increase robustness as histopathology images can look very homogenous and non-histopathology but homogenous pinkish-purple images can fool most classifiers. The ensemble is made up of two small Conv-NeXt model \citep{liu2022convnet} and one linear classifier finetuned with DINO features. The first Conv-NeXt model is trained specifically to detect non-H\&E IHC stained tissue images and the other models are trained on all the IHC stains and tissue types, including on 8 sub-groups of the TCGA WSI dataset and a mix of natural-images, powerpoint(slide) images and scientific figure datasets  (see model, training and data details in section ***). To determine \textbf{(B)} we randomly select $min($num\_of\_predicted\_histo\_scene\_frames $, 20)$ predicted histo scene-frames, and for each selected frame, we extract the next three histo scene-frames and leveraged a pretrained CLIP \footnote{https://huggingface.co/sentence-transformers/clip-ViT-B-32} (ViT-B-32) model to determine the cosine similarity between the selected frame and each of the next three frames, if all three have similarity scores $\geq$ a preset threshold of $0.9$ its counted as one narrative streak. After all selected frames are checked, A video is tagged as narrative style if at least 10\% of the selected frames have a narrative streak. At the end, we then download the high resolution versions of the videos with $\geq 10 \%$ narrative score. 

For \textbf{(A)} we trained a set of binary image classifiers and ensemble their predictions to increase robustness. This ensemble, designed for robustness, comprises two small Conv-NeXt models \cite{liu2022convnet} and one linear classifier fine-tuned with DINO features. Given the homogenous appearance of histopathology images, and the risk of false positives from similar pinkish-purple images, such a combination is necessary. One Conv-NeXt model is trained in detecting non-H\&E IHC stained tissue images, while the other models are trained on all IHC stains and tissue types. These include eight sub-groups of the TCGA WSI dataset and a mix of general-domain images, PowerPoint(slide) images, and scientific figure datasets (see model, training and data details in section x). 


 To identify narrative-style videos \textbf{(B)}, we randomly select a $min($num\_of\_predicted\_histo\_scene\_frames$, 20)$ predicted to be histo scene-frames. For each selected frame, we extract the next three histopathology scene-frames. Utilizing a pre-trained CLIP \footnote{https://huggingface.co/sentence-transformers/clip-ViT-B-32} (ViT-B-32) model, we then compute the cosine similarity between the selected frame and each of the subsequent three frames. If all three have similarity scores $\geq$ a preset threshold of $0.9$ we count it as a narrative streak. A video is identified as narrative style if at least 10\% of the selected frames exhibit a narrative streak. Consequently, we download high-resolution versions of videos with a narrative score of 10\% or higher. Narrative-style videos typically cover whole slide images at various scales. To collect the magnification information, we train a tissue-image-magnification classifier to predict the following three scales: \{(1-10)x, (>10-20)x, (>20)x\}. This provides relevant metadata for downstream pretraining objectives. 

\label{text_denoising}
\subsubsection{Text Modal: Text Extraction through ASR and Text Denoising}
% Ideally, the workflow here would be to (pre)train/finetune a specialized ASR model for the tasks of medical histopathology transcription, however as is the case with a lot of tasks in the medical domain, there aren't any large datasets to utilize, due to its sensitive nature and the cost of acquiring such data with experts. To circumvent this drawback, avoid costly private medical ASR API's, while leveraging open models, we use the Whisper (Large-V2) ASR model. We do not leverage Youtube's ASR caption as it is not available for a lot of videos and in other to maintain homogeneity and promote reproducible for medical ASR transcription we leverage the open-sourced large Version of Whisper \citet{radford2022robust}.

WHAT DOES TEXT MODAL MEAN?

While YouTube's ASR system offers a general solution for natural videos, it falls short of effectively serving the specialized requirements of the medical domain, particularly in the context of histopathology transcription. An ideal approach would be to deploy a specialized ASR model, specifically trained for this task. However, this strategy is constrained by the scarcity of comprehensive datasets, largely due to the sensitive nature of medical data and the costs involved in gathering expert-annotated resources. While there are promising private medical ASR APIs available, their high costs and error-rates render them infeasible. As an alternative, we choose to leverage the open-source Whisper (Large-V2) ASR model \cite{radford2022robust}, with post-processing algorithms to reduce error-rate. As expected, general-domain ASR models like Whisper often incorrectly transcribe medical words/phrases, especially when the speaker's voice is choppy and accented. There are no straightforward trivial solutions due to: \textbf{1)} the absence of openly available medical ASR models or data for fine-tuning in the medical domain; \textbf{2)} the inadequacy of medical named entity recognition models in detecting transcription errors, because these models are typically trained on correctly spelled words; \textbf{3)} the ineffectiveness of methods like semantically searching over a medical glossary, such as the UMLS, which only prove effective when the erroneous text has significant similarity to the correct terms; and \textbf{4)} the inability of simpler methods like finding the longest common substring, which might work in finding a match in the glossary/ontology for replacement, but cannot identify the wrong words/phrases in the first place.

% \begin{enumerate}
%     \item The absence of openly available medical ASR models or data for fine-tuning in the medical domain.
%     \item The inadequacy of medical named entity recognition models in detecting transcription errors, because these models are typically trained on correctly spelled words.
%     \item  Similarly, methods like semantically searching over a medical glossary, such as the UMLS, only prove effective when the erroneous text has significant similarity to the correct terms.
%     \item Simpler methods like finding the longest common substring might work in finding a match in the glossary/ontology for replacement, but the problem of identifying the wrong words/phrases in the first place still persists.
% \end{enumerate}

Given these problems, Whisper requires an additional quality control and correction pipeline to tackle transcription errors. We propose the following text de-noising and quality control pipeline: \textbf{i)} Initially, we employ the Rake keyword extraction algorithm \cite{rose2010automatic}, to extract keywords or key-phrases up to four words in length. After, we further refine these entries (words/phrases) to eliminate those entirely comprised of stopwords, and remove stopwords at the beginning of multi-word entries. \textbf{ii)} We then cross-checked each refined entry against the UMLS database using the SciSpacy entity linking package \cite{neumann-etal-2019-scispacy}. If an entry is not found within the UMLS, we check for misspelled words within the entry using a spell-checking algorithm\footnote{https://github.com/barrust/pyspellchecker}, instantiated with a specialized list of histopathology terms that curated from various histopathology ontology labels and definitions. Qualitatively this process ensures high precision albeit at lower recall (see example in Supplement****). \textbf{iii)} With this probable list of misspelled keywords, we condition and prompt the LLM (GPT-$3.5$) with examples to correct the misspelled entry within its context(sentence), and identify additional missed errors/misspelled entries (see Figure \ref{fig:asr_cor_fig}). For more examples and failure cases see  Appendix WHATEVER***. \textbf{iv)} Finally, to de-noise the text, we resolve the output mapping of incorrect $\mapsto$ correct entries by verifying the corrected words against UMLS and our curated list of histopathology words/phrases. Entries that pass this double-validation process are used to replace the initial noisy transcription.


% \begin{enumerate}[label=(\roman*)]
 
%     \item Initially, we employ the Rake keyword extraction algorithm \citet{rose2010automatic}, to extract keywords or key-phrases up to four words in length. After, we further refine these entries (words/phrases) to eliminate those entirely comprised of stopwords, and remove stopwords at the beginning of multi-word entries.
    
%     \item We, then cross-checked each refined entry against the UMLS database using the SciSpacy entity linking package \citet{neumann-etal-2019-scispacy}. If an entry is not found within the UMLS, we check for misspelled words within the entry using a spell-checking algorithm\footnote{https://github.com/barrust/pyspellchecker}, instantiated with a specialized list of histopathology terms that curated from various histopathology ontology labels and definitions. Qualitatively this process ensures high precision albeit at lower recall (see example in Supplement****)
    
%     \item With this probable list of misspelled keywords, we condition and prompt the LLM (GPT-$3.5$) with few-examples to correct the misspelled entry within its context(sentence), and identify additional missed errors/misspelled entries (see Figure \ref{fig:asr_cor_fig}). For more examples and failure cases see  Appendix WHATEVER***.

%     \item Finally, to de-noise the text, we resolve the output mapping of incorrect $\mapsto$ correct entries by verifying the corrected words against UMLS and our curated list of histopathology words/phrases. Entries that pass this double-validation process are used to replace the initial noisy transcription.
    
% \end{enumerate}


Leveraging domain-specific databases to extract the text and filter out the noise allows us to bypass the correction of repetition errors and filler words, such as \textit{'ah', 'uhm', or 'the the' etc.} in tandem, using LLMs (GPT $3.5$) allows us to concentrate on correcting medically relevant misspelled words, rather than wasting compute on correcting non-medically relevant terms. 

\label{med_text_ext}
\subsubsection{Medical Text Extraction}

To filter relevant medical text and Region of Interest (ROI) text from the ASR-corrected text, we once again utilize LLMs. This decision is rooted in two compelling reasons:

\begin{enumerate}
    \item At scale, and especially for tasks like curating pre-training datasets that can tolerate a certain level of noise, LLMs can be more cost-effective than human labor.

    \item Moreover, the tasks does not require LLMs to generate new information but instead to discriminate useful versus irrelevant signals, serving to improve the signal-to-noise ratio of the data by extracting and highlighting relevant information.
\end{enumerate}


To extract relevant text, we prompt LLMs to filter out all non medically-relevant text, providing context as necessary. Lastly, we instruct the LLMs to refrain from introducing any new words beyond the corrected noisy text by setting the model's temperature to zero (see Figure \ref{fig:asr_cor_fig}). More details about the prompt used and additional examples can be found in Appendix ***.

Finally, we use LLMs to categorize our videos into one of the 18 identified sub-pathology classes. Similar to the previous tasks, this categorization is done by conditioning with few examples and prompting the LLM to predict the top three possible classes given the text.



\subsubsection{Image Modal: Image Extraction and Denoising} 
\label{img_modal}

%new
% For each video, we employ a similar method described in \ref{search_filter} to extract histopathology scene-frames, our method leverages these frame's time $t$ as beacons to chunk the entire video (see \ref{chunking}) into time-intervals to extract representative images from. Next, for each chunk $(t_n, t_{n+1})$, we use the static chunk detection algorithm described in \ref{algo1} to extract sub-time-intervals with static frames within the chunk, if found we save the median (in pixel space to prevent blurry outputs) of the stable frames, else we leverage structural similarity index (SSIM) method on scene-frames to find the most dissimilar histopathology image to makeup the representative images for the chunk, see Figure \ref{fig:image_denoising}. In essence, we use the histopathology scene frames as guides where to collect data in the video, and then we exploit the human behaviour of pausing while narrating in an educational video to explain by using our stable-detection algorithm to find those chunks of time and extract the median frame, for chunks where we don't find these stable regions we simply revert back to the histopathology scene-frames (beacons) and only take the most representative frames by removing duplicates.

For each video, we employ a similar method to that described in \ref{search_filter} to extract histopathology scene-frames; our method leverages these frames' times $t$ as beacons to break the entire video (see \ref{chunking}) into time-intervals from which to extract representative images. Next, for each chunk $(t_n, t_{n+1})$, we use the static chunk detection algorithm \ref{algo1} (described in supplementary material)  to extract sub-time-intervals with static frames within the chunk. If found we save the median (in pixel space to prevent blurry outputs) of the stable frames, else we leverage the structural similarity index (SSIM) method on scene-frames to find the most dissimilar histopathology image to make up the representative images for the chunk see Figure \ref{fig:image_denoising}). In essence,  we use the extracted histopathology scene frames as guides for data collection points within the video.  Then we exploit the human tendency in educational videos to pause narration during explanation, using our stable chunk detection algorithm to locate these pause points and extract the median frame. For chunks without stable regions, we rely on the initial histopathology scene-frames (beacons) and filter out duplicate frames to ensure only the most representative frames are retained. ARE YOU LOOKING FOR ONE OR SEVERAL FRAMES PER CHUNK? STATE THE GOAL FIRST.

%old
%We utilize video frames to extract images and we consider various aspects of each frame, such as its dissimilarity to neighboring frames and the presence of a stable background. Many videos in our dataset contain noise from video editing or artifacts introduced by the software used for WSI viewing. To extract stable frames, we measure the absolute difference between consecutive frames. Typically, the histopathology parts of the image change slightly across frames, while the artifacts remain consistent. We determine the representative image for each video chunk by calculating the median (in pixel space) of the stable frames. If a stable background is not found, we calculate Structural Similarity Index (SSIM) between these images and only keep the most dissimilar images. Algorithm \ref{algo1} and  provides a detailed description of how we select and extract images for our dataset.


\subsubsection{Aligning All Modalities}
\begin{figure}[ht!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}width=0.8\linewidth, 
\includegraphics[width=1\linewidth]{resources/images/alignment_fig.pdf}
\end{center}
   \caption{\textbf{An overview of our proposed dataset target and source formats} NEEDS MORE EXPLANATION}
\label{fig:alignment}
\end{figure}

For each narrative-style video, we perform the following steps to align image and text modalities:

\begin{enumerate}
    \label{chunking}
    \item First, we compute histopathology time chunks denoted as $[(t_1, t_2), (t_3, t_4), \cdots (t_{n-1}, t_n)]$ from scene frames after discriminating histopathology frames using the histopathology ensemble classifier -- (\textit{scene\_chunks}). Each \textit{scene\_chunk} is padded with \textit{pad\_time} to its left and right; see Figure \ref{fig:histo_chunking} and Table \ref{tab:histo_chunk} for more details.

    \item \textbf{Text:} we use the ASR output to extract the words spoken during each chunk in \textit{scene\_chunks}. Using the method descried in \ref{med_text_ext}, we extract the Medical and ROI caption for this chunk.

    \item \textbf{Image:} we extract representative image(s) for every chunk/time-interval in \textit{scene\_chunks} as described in section \ref{img_modal}
    
    %\begin{enumerate}
    %    \item We use the method described in \ref{img_modal} to find time-intervals within each chunk with stable background/frames. If such frames are found we extract the median (in pixel space) image(s) from these regions. 
    %    \item If not we leverage the histopathology scene frames in the chunk and reduce the number of scene frames by finding the most dissimilar set of frames. 
    %\end{enumerate}


    \item At this point each chunk in \textit{scene\_chunks} is mapped to texts (both medical and ROI captions) and images. Next we map each medical image to one or more medical text extracted using the method described in \ref{med_text_ext}.
    
    \begin{enumerate}
        \item Using the time interval of which the image occurs in, we extract its raw text from ASR and then correct and extract keywords using the Rake method, and we refer to these as \textit{raw\_keywords}.
        
        \item We extract keywords from each medical text in the list of medical image texts returned using the LLM, and we refer to these as \textit{keywords}.
        
        \item Finally, we map each medical text whose \textit{keywords} overlap with \textit{raw\_keywords}; see Figure \ref{fig:alignment}.I DON'T GET THIS, NEEDS AN EXAMPLE FIG 3 USELESS.
    \end{enumerate}

\end{enumerate}


These steps complete the many-to-many mapping and alignment of the dataset modalities. By stacking these chunks of data, we can represent an entire video and its procedural nature.

%------------------------------------------------------------------------------------------------
\begin{figure}[ht!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}width=0.8\linewidth, 
\includegraphics[width=0.8\linewidth]{resources/images/histo_chunk_fig.pdf}
\end{center}
   \caption{\textbf{Image-Text time chunking algorithm} Diagram representing how we chunk images and text from videos. Each Transition Tag is described in Table \ref{tab:histo_chunk} THIS FIGURE NEEDS A LOT MORE EXPLANATION or delete.
   }
\label{fig:histo_chunking}
\end{figure}
%------------------------------------------------------------------------------------------------

%------------------------------------------------------------------------------------------------


\begin{figure}[ht!]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}width=0.8\linewidth, 
\includegraphics[width=\linewidth]{resources/images/asr_med_roi_fig.pdf}
\end{center}
   \caption{\textbf{in the blue and yellow we highlight ...THIS IS TOO SMALL TO READ}}
\label{fig:asr_cor_fig}
\end{figure}



%-------------------------------------------------------------------------


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


